Unsplittable Flow on a Short Path

In the Unsplittable Flow on a Path problem UFP, we are given a path graph with edge capacities and a collection of tasks. Each task is characterized by a demand, a profit, and a subpath. Our goal is to select a maximum profit subset of tasks such that the total demand of the selected tasks that use each edge $e$ is at most the capacity of $e$. Bag-UFP is the generalization of UFP where tasks are partitioned into bags, and we are allowed to select at most one task per bag. UFP admits a PTAS [Grandoni,M{\"o}mke,Wiese'22] but not an EPTAS [Wiese'17]. Bag-UFP is APX-hard [Spieksma'99] and the current best approximation is $O(\log n/\log\log n)$ [Grandoni,Ingala,Uniyal'15], where $n$ is the number of tasks. In this paper, we study the mentioned two problems when parameterized by the number $m$ of edges in the graph, with the goal of designing faster parameterized approximation algorithms. We present a parameterized EPTAS for Bag-UFP, and a substantially faster parameterized EPTAS for UFP (which is an FPTAS for $m=O(1)$). We also show that a parameterized FPTAS for UFP (hence for BagUFP) does not exist, therefore our results are qualitatively tight.

==> VKhardness.tex <==
In this section, we give the hardness of the VK problem as stated in \Cref{thm:VK_app_hardness}. 


\begin{proof}[Proof of \Cref{thm:VK_app_hardness}]
	We give a reduction from the $k$-{\em independent set problem}. In this problem, we are given a pair $(G,k)$ where $G = (V,E)$ is a graph and $k \in \mathbb{N}$ is a parameter. A solution is an independent set in $G$ with at most $k$ vertices. The goal is to find a maximum cardinality solution. Let $I = (G,k)$, where $G = (V,E)$ be a $k$-independent set instance. Define the {\em reduced} VK instance of $(G,k)$ as the tuple $R = (V,E,c,w,u)$ such that the following holds.  For every $v \in V$ and $e \in E$ define $c_e(v) = 1$ if $v$ is an endpoint of $e$; otherwise, define $c_e(v) = 0$. Moreover, for all $e \in E$ and $v \in V$ define $u(e) = 1$ and $w(v) = 1$. %The cost function $c:V \rightarrow \mathbb{R}_{\geq 0}$
	
	By the above, some $S \subseteq V$ is an independent set in $G$ if and only if for all $e \in E$ it holds that $$\sum_{v \in S} c_e(v) = \left|\left\{ v \in S~|~\textnormal{$v$ is an endpoint of $e$ } \right\}\right| \leq 1 = u(e).$$
	Therefore, for every $0 \leq q \leq k$, $I$ has a solution of size $q$ if and only if $R$ has a solution of weight $q$ (the weights are uniform in $R$). Hence, under \textnormal{Gap-ETH} and by the hardness results of \cite{chalermsook2017gap} on $k$-independent set, the statement follows.  %if the statement of the lemma does not hold, 
	%Clearly, for every $1 \leq q \leq k$, there is an independent set in $G$ of cardinality $q$ if and only if there is a solution for $R$: 
\end{proof}


==> preliminaries.tex <==




Given an instance $I$ of a \fab{maximization} problem \fab{$\Pi$}, let $|I|$ be the encoding size of $I$. 
Let $\OPT(I)$ be the value of an optimal solution for $I$. For $\alpha \in (0,1]$, we say that $S$ is an $\alpha$-approximate solution for instance $I$ if $S$ is a solution for $I$ of value at least $\alpha \cdot \OPT(I)$. 


A\fabr{Rephrased a bit, old version commented} Polynomial-Time Approximation Scheme (PTAS) for $\Pi$ is a family of algorithms $(A_{\eps})_{\eps>0}$ such that, for any $\eps>0$, $A_{\eps}$ returns a $(1 - \eps)$-approximate solution in time $|I|^{g\left(\frac{1}{\eps}\right)}$, where $g$ is a computable function. An Efficient PTAS or EPTAS (resp., Fully PTAS or FPTAS) is a PTAS where the running time is of the form $g\left(\frac{1}{\eps}\right) \cdot |I|^{O(1)}$ (resp., $\left(\frac{|I|}{\eps}\right)^{O(1)}$).

For a given parameter $k$ of the input, a Parameterized PTAS (\pP) is defined similarly to a PTAS with the difference that there is an extra multiplicative factor $f(k)$ in the running time, where $f$ is a computable function, namely the running time is of the form $f(k)\cdot |I|^{g\left(\frac{1}{\eps}\right)}$. Similarly in a \pE\ (resp., \pF) the running time is of the form $f(k)\cdot g\left(\frac{1}{\eps}\right) \cdot |I|^{O(1)}$ (resp., $f(k)\cdot \left(\frac{|I|}{\eps}\right)^{O(1)}$).

